Generating Visual Representations for Zero-Shot Classification

This paper addresses the task of learning an image clas-sifier when some categories are defined by semantic descriptions only (e.g. visual attributes) while the others are defined by exemplar images as well. This task is often referred to as the Zero-Shot classification task (ZSC). Most of the previous methods rely on learning a common embedding space allowing to compare visual features of unknown categories with semantic descriptions. This paper argues that these approaches are limited as i) efficient discrimi-native classifiers can't be used ii) classification tasks with seen and unseen categories (Generalized Zero-Shot Classification or GZSC) can't be addressed efficiently. In contrast , this paper suggests to address ZSC and GZSC by i) learning a conditional generator using seen classes ii) generate artificial training examples for the categories without exemplars. ZSC is then turned into a standard supervised learning problem. Experiments with 4 generative models and 5 datasets experimentally validate the approach, giving state-of-the-art results on both ZSC and GZSC.

==> 4-related_work.tex <==
\section{Related works}
\label{sec:related_work}
\paragraph{Zero-Shot Classification} 
First studies tackle ZSC as an attribute detection problem. \cite{Lampert:2014fs} introduced the  Direct Attribute Prediction  method, based on independent attribute detectors used to build an image embedding. In this case, the similarity score is simply the conditional probability of a class given the image. \cite{farhadi2009describing} developed a similar approach, where the score function is based on the Euclidean distance. These two approaches do not model attribute correlations nor any relative importance between them.
To overcome these limitations, and inspired by \cite{weston2011wsabie}, most of the recent works such as \cite{Akata:2015tv,Frome:2013ux,romera2015embarrassingly,xian2016latent} address ZSC as an embedding problem. They learn two mapping functions, projecting image data and class descriptions into a common semantic space in which their similarity can be measured through a consistency function. \cite{Akata:2015tv} proposed a bilinear function for measuring the similarity between images and class descriptions, optimized to ensure a higher ranking of compatible image-class pairs. 
\cite{xian2016latent} improved the embedding function by introducing latent variable, allowing the selection of the map to use for a specific image-class pair. \cite{romera2015embarrassingly} solved ZSC as a closed form solution assuming a specific form of regularization. 
\cite{changpinyo2016synthesized} proposed a manifold-based approach  aligning the semantic and image space with the use of phantom classes. \cite{zhang2016zero} modeled the posterior probability of a match and propose a latent probabilistic model in this context. They jointly learn the parameters of their model for both domains, which ultimately leads to class-independent classifiers.
\cite{Zhang:2015vs} represented unseen classes as a mixture of seen classes proportions, with classification decisions following the seen class similarity patterns.
\cite{Bucher:2016tv,bucher2016hard} proposed to improve and transform the attribute space by the use of a metric learning approach. The learning procedure optimizes both the embedding and the metric in a multi-objective criterion formulation.
Lastly, works such as \cite{Frome:2013ux,norouzi2013zero}  introduced a large-scale version of ZSC, where classification evaluation is done on the ImageNet dataset \cite{deng2009imagenet}.
Compared to traditional ZSC datasets, ImageNet is more challenging with more unseen classes than seen ones (1000 vs. 20,842) as well as a larger number of classes ($\approx$22000).
Recently, \cite{chao2016empirical} introduced the Generalized Zero-Shot Learning (GZSL) task, a more realistic task where,  at test time, images from both seen and unseen classes have to be classified. \cite{chao2016empirical} have shown that traditional approaches suffer from bias decision issues in this new scenario. To tackle this problem, the authors proposed to penalize the score of seen classes.


\paragraph{Generation of training examples}

\cite{Guo:2004dh} noticed that learning from imbalanced data sets, where the number of examples of one (majority) class is much higher than the others, presents an important challenge to the machine learning community.  Since then, several works addressed the question of generating novel training example from existing ones, when the training sets are unbalanced. Using a bootstrapping process,  \cite{Melville:2003us} generated artificial training data by randomly picking data points from an approximation of the training-data distribution. They compute the mean and standard deviation of numeric attributes from the training set and generate values from the Gaussian distribution defined by these. \cite{BaderElDen:2016du} extended the popular SMOTE (Synthetic Minority Over-sampling Technique) technique, which generates new synthetic minority instances created from a chosen point of the line that links the selected instance to its nearest minority neighbor. Generating novel training examples from the existing ones is also at the heart of the technique called {\em Data Augmentation}, frequently used for training deep neural networks \cite{LeCun:1998hy}.  

The aforementioned techniques can't be used when there is no training data at all for some categories. However, in these situations, if some underlying parametric representation of the data can be obtained, it can be used to generate novel training data, assuming a mapping from the underlying representation to the image space. \cite{Eggert:2015ia} explores this strategy by synthetically generating data for the task of company logo detection with deep-learned features in the absence of a large training set. Synthetically generated images are obtained by applying warping and other geometric / photometric transformations to prototypical logo exemplars. A similar idea was also presented in \cite{jaderberg2015reading} for text spotting in images. In \cite{Cabrera:2016ix} the authors first capture what they call {\em The Gist of a Gesture} by recording human gestures, representing them by a model and using this model to generate a large set of realistic gestures. 

We build in this direction for ZSC, the underlying representation being some attribute or text based description of the unseen categories, and the transformation from attributes to image features being learned from the examples of the seen classes. A relevant way to learn this transformation is to use generative models such as  {\em denoising auto encoders} \cite{bengio2013generalized} and {\em generative adversarial nets} \cite{Goodfellow:2014td} or their variants \cite{Che:2016wq,makhzani2015adversarial}. GANs consist in estimating generative models via an adversarial process simultaneously training two models,  a generative model that captures the data distribution, and a discriminative model that estimates the probability that a sample came from the training data rather than the generator. 
